From Boltzmann Machines to Neural Networks and Back Again

Graphical models are powerful tools for modeling high-dimensional data, but learning graphical models in the presence of latent variables is well-known to be difficult. In this work we give new results for learning Restricted Boltzmann Machines, probably the most well-studied class of latent variable models. Our results are based on new connections to learning two-layer neural networks under $\ell_{\infty}$ bounded input; for both problems, we give nearly optimal results under the conjectured hardness of sparse parity with noise. Using the connection between RBMs and feedforward networks, we also initiate the theoretical study of $supervised~RBMs$ [Hinton, 2012], a version of neural-network learning that couples distributional assumptions induced from the underlying graphical model with the architecture of the unknown function class. We then give an algorithm for learning a natural class of supervised RBMs with better runtime than what is possible for its related class of networks without distributional assumptions.

==> files/intro.tex <==
Graphical models are a powerful framework for modelling high-dimensional distributions in a way that is interpretable and enables sophisticated forms of inference and reasoning. They are extensively used in a variety of disciplines including the natural and social sciences where they have been used to model the structure of gene regulatory networks, of connectivity in the brain, and the flocking behavior of birds \citep{bialek2012statistical}. In many contexts, the structure of interactions between different observed variables is unknown a priori and the goal is to infer this structure in a sample-efficient way from data. There has been decades of research on various formulations of this problem, both theoretically and empirically: for example, provable algorithms have been developed for learning tree-structured graphical models \citep{ChowL}, for learning models on graphs of bounded tree-width \citep{karger2001learning}, for learning Ising models on general graphs of bounded degree \citep{BreslerMosselSly,Bresler,Vuffray,KlivansM} and in a variety of other contexts like Gaussian graphical models (e.g. \cite{meinshausen2006high}). For the most part, the main interest has been on learning under the assumption that the underlying model is sparse. Sparsity is a natural assumption since many applications are in a sample-starved regime where the learning problem is information-theoretically impossible without sparsity. Sparse models are generally considered to be more interpretable than their dense counterparts since they satisfy large numbers of conditional independence relations.
%in terms of provable algorithms, a seminal work in 1968 of \cite{ChowL} for provably learning tree-structured graphical models, works on learning \cite{karger2001learning}

A major challenge in probabilistic inference from data is the presence of latent or confounding variables which are unobserved and may create complicated higher-order dependencies between the observed variables. Specifically in the context of learning undirected graphical models, it is well known that even if the underlying graphical model is well-behaved, if only a subset of the variables are observed then the resulting marginal distribution can still be extremely complicated, e.g. simulating the uniform distribution over satisfying assignments of an arbitrary circuit \citep{BogdanovMV}, which makes the learning problem computationally intractable. On the other hand, under certain assumptions we know that learning graphical models with latent variables can be both computationally and statistical tractable; for example, the setting of tree-structured models with latent variables has been extensively studied in the context of phylogenetic reconstruction, see e.g. \citep{felsenstein2004inferring,daskalakis2006optimal}. However, in non-tree-structured models there are comparatively few positive results for recovering latent variable models in a computationally efficient fashion. One of the few exceptions is in the Gaussian case, where \cite{ChandrasekaranPW} gave a positive result; this setting is very special, as latent variable GGMs \emph{do not} have higher-order interactions, but in fact are equivalent to GGMs with cliques.

In this work, we will focus on a latent variable model popularized in the neural network literature known as the \emph{Restricted Boltzmann Machine} (RBM) (see e.g. \cite{hinton2012practical,goodfellow2016deep}) which has been applied to problems such as dimensionality reduction and collaborative filtering \citep{RBMdimension,RBMclassification,RBMfeature}. It is also perhaps the most canonical version of an Ising model with latent variables.
The RBM describes a joint distribution over observed random variables $X$ valued in $\{\pm 1\}^{n_1}$ and latent variables $H$ valued in $\{ \pm 1\}^{n_2}$
\begin{align*} \Pr(X = x,H = h) \propto \exp\left(\langle x, Wh \rangle + \langle b^{(1)}, x \rangle + \langle b^{(2)}, h \rangle \right) \end{align*}
where the \emph{weight matrix} $W$ is an arbitrary $n_1 \times n_2$ matrix and \emph{external fields}/\emph{biases} $b^{(1)} \in \mathbb{R}^{n_1}$ and $b^{(2)} \in \mathbb{R}^{n_2}$ are arbitrary, and $X$ is referred to as the vector of \emph{visible unit} activations and $H$ the vector of \emph{hidden unit} activations. In the learning problem, we are given access to i.i.d. samples of $X$ but do not get to observe $H$. It is not hard to see that in the special case where the hidden nodes are constrained to have degree 2, the class of marginal distributions on $X$ induced by RBMs is exactly the class of Ising models (pairwise binary graphical models), so the general RBM can be thought of as a natural generalization of fully-observed Ising models, for which the learning problem is well-understood. We also note that the parameters of the RBM are not identifiable even given an infinite number of samples, so our goal for learning the RBM is generally speaking to learn the distribution or related structural properties (e.g. the Markov blankets of the nodes in $X$).

In recent work \citep{bresler2019learning,goel2019learning}, the first provable algorithms were developed for learning RBMs, under the assumptions that the model is (1) sparse and (2) ferromagnetic. On the other hand, it was shown in \citep{bresler2019learning} that learning general sparse RBMs is computationally intractable in general, because the conjecturally hard problem of learning a \emph{sparse parity with noise} can be embedded into a sparse RBM with a constant number of hidden units. The assumption of ferromagneticity (that variables are only positively correlated, not negatively correlated) rules out this example and plays a crucial role in the analysis of these works. Without ferromagneticity, viewing $X$ as the observed distribution of a general Markov Random Field allows for using prior work \cite{KlivansM} to give learning algorithms with runtime $n^{O(d_H)}$ where $d_H$ is the maximum degree of a hidden node. This matches the lower bound of learning sparse parity with noise mentioned previously.

To summarize, the best previous results for learning RBMs either (1) make the assumption of ferromagneticity which makes building sparse parities impossible or (2) ignore all of the structure of the RBM except the max hidden degree, and pay the price of a $n^{\Theta(d_H)}$ runtime. This leaves open the question of developing algorithms whose runtime depends on some natural notion of a \emph{complexity} measures of the RBM.

In this paper, we design an algorithm that is adaptive to a {\em norm} based complexity measure of the RBM, and often outperforms approach (2) above significantly, while not eliminating the possibility of negative correlation completely as in (1). 
%restricting the class of models considered. 
The key idea of our approach is to develop a novel connection between learning RBMs and their historical relative, feedforward neural networks. This connection allows us to establish new results for learning RBMs via proving new results about learning feedforward neural networks. Our connection also validates the idea of a so-called {\em supervised RBMs} as a natural distributional setting for classification with feedforward networks. Supervised RBMs, proposed by \citet{hinton2012practical}, treat one visible unit of the RBM as the label and the other visible units as the input to the classifier. This allows us to use the
% the optimal predictor is a feedforward network
 connection in the ``reverse'' direction --- using natural structural assumptions on the RBM (like ferromagneticity) to give better results for solving supervised prediction tasks in an interesting distributional setting. Along these lines, we show that an assumption related to ferromagneticity, but allowing for some amount of negative correlation in the RBM, allows us to learn the induced feedforward network faster than would be possible without distributional assumptions.
%After establishing a new result for learning RBMs, we also show how to use this connection in the ``reverse'' direction. 
%: under some assumptions which make the RBM behave nicely, when the input data is generated from the corresponding RBM we show how to learn feedforward networks using RBM learning as a subroutine faster than would be possible without distributional assumptions.

\paragraph{Our Results}
% \section{Learning RBMs via New Results for Feedforward Networks}
% \begin{defn} \label{def:rbm}
% A \emph{Restricted Boltzmann Machine} is any joint distribution over random variables $X$ valued in $\{\pm 1\}^{n_1}$ and $H$ valued in $\{ \pm 1\}^{n_2}$ of the form
% \[ \Pr(X = x,H = h) = \frac{1}{Z} \exp\left(\langle x, Wh \rangle + \langle b^{(1)}, x \rangle + \langle b^{(2)}, h \rangle \right) \]
% where the \emph{weight matrix} $W$ is an arbitrary $n_V \times n_H$ matrix and \emph{external fields}/\emph{biases} $b^{(1)} \in \mathbb{R}^{n_1}$ and $b^{(2)} \in \mathbb{R}^{n_2}$ are arbitrary, and 
% $X$ is referred to as the vector of \emph{visible unit} activations and $H$ the vector of \emph{hidden unit} activations.
% \end{defn}
Our first result characterizes the relationship between RBMs and Feedforward networks. We show that there is a natural self-supervised prediction task in RBMs, of predicting the spin at node $i$ given all other observed nodes, for which the Bayes-optimal predictor is \emph{exactly given} by a two-layer feedforward network with a special family of $\tanh$-like activations.
\begin{theorem}[Informal version of Theorem~\ref{thm:node-prediction}]\label{thm:node-prediction-intro}
For any visible unit $i$ in an arbitrary RBM,
%\[ \E[X_i | X_{\sim i}] = \tanh\left(b^{(1)}_i + \sum_j \tanh^{-1}\left(\tanh(W_{ij})\tanh\left(b^{(2)}_j + \sum_{k \ne i} W_{kj} X_k\right)\right)\right) \]
\begin{equation*}%\label{eqn:node-prediction} 
\E[X_i | X_{\sim i}] = \tanh\left(b^{(1)}_i + \sum_j \tanh(W_{ij}) f_{\beta_{ij}}\Big(b^{(2)}_j + \sum_{k \ne i} W_{kj} X_k\Big)\right) 
\end{equation*}
where $\beta_{ij} = |\tanh(W_{ij})|$ and $f_{\beta}(x) := \frac{1}{\beta} \tanh^{-1}(\beta \tanh(x))$.
\end{theorem}
The activations $f_{\beta}$ in this network naturally interpolate between $\tanh$ at $\beta = 0$ and linear at $\beta = 1$, see Remark~\ref{rmk:f-activation}.
The exact structure of this prediction function is crucial in what follows and does not seem to have been known in the RBM literature, though some related ideas have been used to develop better heuristics for performing inference and training in RBMs (see discussion in Section~\ref{sec:connections}). 

Given this connection, we show that if we can solve the problem of learning such a neural network within sufficiently small error, then we can successfully learn the RBM. This reduces our RBM learning problem to that of learning feedforward neural networks in the setting that the input is bounded in $\ell_{\infty}$ norm.  %We state first the results that this ultimately gives for structure learning in RBMs.

%This result is proved based upon a result for learning the corresponding feedforward networks which is 
Subsequently, we give results for the feedforward network problem which are
nearly optimal both in the terms of sample complexity (in the regime where $\lambda$ is bounded) and in terms of computational complexity under the hardness of learning sparse parity with noise; some aspects of this result are new even for the well-studied case of learning neural networks with $\tanh$ activations (see Further Discussion).% \fnote{is this true?} \snote{Unclear since this setup was not considered ($L_\infty$ bounded input, I mean)} 
\begin{theorem}[Informal version of Corollary~\ref{corr:rbm-regression-simple}]\label{thm:regression-intro}
Suppose that $Y$ is a random variable valued in $\{\pm 1\}$, $X$ is a random vector such that $\|X\|_{\infty} \le 1$ almost surely and
\[ \E[Y | X] = \tanh\left(b^{(1)} + \sum_j w_j f_{\beta_j}\Big(b^{(2)}_j + \sum_{k} W_{jk} X_k\Big)\right) \]
where $b^{(1)} \in \mathbb{R}$, $\beta_j \in [0,1]$, $w$ is an arbitrary real vector and $W$ is an arbitrary real matrix. Let $W_j$ denote \emph{column} $j$ of $W$ and suppose $\|W_j\|_1 \le \lambda$ for every $j$ and some $\lambda \ge 2$. Then if we run $\ell_1$-constrained regression on the degree $D$ monomial feature map $\varphi_D(x) \mapsto \left(\prod_{i \in S} X_i\right)_{|S| \le d}$ with appropriate $\ell_1$ constraint, the result $\hat{w}$ satisfies with high probability
\[ \E[\ell(\hat{w} \cdot \varphi_d(X), Y)] \le OPT + \epsilon \]
where $OPT$ is the minimum logistic loss for any measurable function of $X$,
as long as the number of samples $m$ satisfies $m = \Omega((|b^{(1)}|^2 \lambda^{O(D)})\log(2n))$ where $D = O(\lambda \log(\|w\|_1\lambda/\epsilon))$ and the runtime of the algorithm is $poly(n^D)$.
\end{theorem}
We also show, under the standard assumption for hardness of learning sparse parity with noise, that the runtime guarantee in this result is close to tight even in the usual setting of $\tanh$ neural networks ($\beta_j = 0$) --- it is optimal up to $\log \log$ factors in the exponent in its dependence on $\epsilon$ and $\|w\|_1$, and we also show that at least a subexponential dependence (essentially $2^{\sqrt{\lambda}}$) on $\lambda$ is unavoidable (assuming the dependence on other parameters in the statement is fixed, since there are e.g. trivial algorithms that run in time $2^n$). This result is Theorem~\ref{thm:net-hardness}. To our knowledge, the fact that $n^{\log(\|w\|_1/\epsilon)/\log\log(\|w\|_1/\epsilon)}$ runtime is required to learn this class even for $\lambda = 1$, and by the above upper bound is tight up to the $\log \log$ term, was not known before even for standard $\tanh$ networks. As far as the dependence on $\lambda$, a similar problem was studied in \cite{shalev2011learning} where they proved the dependence cannot be polynomial using the result of \cite{klivans2009cryptographic} for intersection of halfspaces, based on a different assumption, though our lower bound seems to be somewhat stronger in the present context.

In particular the lower bounds on the runtime show that methods like the kernel trick cannot significantly improve the runtime compared to the simple method of writing out the feature map explicitly used in Theorem~\ref{thm:regression-intro}; however, writing out the feature map lets us use $\ell_1$ regularization\footnote{Interestingly, recent work \citep{woodworth2019kernel} has shown in a special case connections between the implicit bias of gradient descent in feedforward networks and $\ell_1$ regularization in function space.} instead of $\ell_2$ which can give significant sample complexity advantages (e.g. $O(\log n)$ vs $O(n)$ for the usual sparse linear regression setups). 
%These results hold for a general distribution of inputs to the network, but are close to tight even in the case studied in our reduction, where the input and output are all visible nodes in a single close to RBM. This shows that in general, assuming the data is generated from a corresponding RBM does not make the problem of learning the feedforward network significantly easier.

\paragraph{Structure learning results: }
As explained above, our reduction based on Theorem~\ref{thm:node-prediction-intro} lets us use the above feedforward network learning result to learn the structure of RBMs. By structure learning, we mean learning the \emph{Markov blanket} of the each visible unit in the marginal distribution of the RBM over visible units, i.e. the minimal set of nodes $S$ such that $X_i$ is conditionally independent of all other $X_j$ conditionally on $X_S$. We will also refer to the Markov blanket as the (two-hop) neighborhood of node $i$.
This is a natural objective as other tasks such as distribution learning are straightforward in sparse models if the Markov blankets are known.
As in the previous work on structure learning in other undirected graphical models (e., we will need some kind of quantitative nondegeneracy condition to guarantee nodes in the Markov blanket of node $i$ are information-theoretically discoverable; it is not hard to see (e.g. using the bounds from \cite{santhanamW}) that if two nodes are neighbors but their interaction is extremely weak then it becomes impossible to distinguish the model from the same model with the edge removed without a very large number of samples. 

In Ising models and in ferromagnetic RBMs, there are simple conditions on the weight matrices which can ensure neighbors are information-theoretically discoverable. 
In a general RBM, there is no natural way to place constraints on the weights of the RBM to ensure this: the issue is that two nodes $X_i$ and $X_j$ can be independent even though they have two neighboring hidden units with non-negligible edge weights, since the effect of those hidden units can exactly cancel out so that $X_i$ and $X_j$ are independent or indistinguishably close to independent (a number of examples are given in \cite{bresler2019learning}). For this reason, we will instead make the following assumption on the behavior of the model itself instead of on its weight matrix:
\begin{defn}
We say that visible nodes $i,j$ are $\eta$-nondegenerate two-hop neighbors if 
\[ \E[\ell(\E[X_i | X_{\sim \{i,j\}}], X_i)] - \E[\ell(\E[X_i | X_{\sim i}], X_i)] \ge \eta \]
or if the same inequality holds with $i$ and $j$ interchanged. %We say the nodes are $\eta$-degenerate neighbors if they are not $\eta$-nondegenerate.
\end{defn}
\begin{example}\label{example:ising-eta}
It is not hard to see that Ising models are equivalent to the marginal distribution of RBMs with maximum hidden node degree equal to $2$. Consider an Ising model with minimum edge weight $\alpha$ and such that the maximum $\ell_1$-norm into every node is upper bounded by $\lambda$ and the external field is upper bounded by $B$, then $\eta \ge e^{-O(\lambda + B)}/\alpha$, see e.g. \cite{Bresler}.
\end{example}
\begin{example}
In a ferromagnetic RBM with minimum edge weight $\alpha$ and maximum external field $B$, it can be shown that $\eta \ge e^{-O(\lambda_1 + \lambda_2 + B)}/\alpha^2$ (see \cite{bresler2019learning,goel2019learning}).
\end{example}

In order for the RBM to be learnable with a reasonable number of samples (since general RBMs can represent arbitrary distributions), we need to assume it is low complexity in the following sense, as alluded to before: 
\begin{defn}
We say that an RBM is $(\lambda_1,\lambda_2)$-bounded if for any $i$, $\sum_j |\tanh(W_{ij})| + |b^{(1)}_i| \le \lambda_1$ and the columns of $W$ are bounded in $\ell_1$ norm by $\lambda_2$. %Note that $\lambda_1$ bounds the $\ell_1$ norm into 
%(As we will see, $\lambda_1$ and $\lambda_2$ actually play very different roles when it comes to the difficulty of learning the RBM.)
\end{defn}
Note that $\lambda_1$ essentially bounds the $\ell_1$ norm into visible units, and $\lambda_2$ the $\ell_2$ norm into hidden units. Based on our upper bounds and lower bounds for the learnability of feedforward networks, it should be less surprising that these parameters play a very different role in the computational learnability of RBMs.
\begin{theorem}[Informal version of Theorem~\ref{thm:rbm-structure-recovery}]\label{thm:rbm-structure-recovery-informal}
Suppose all two-neighbors in a $(\lambda_1,\lambda_2)$-bounded RBM are $\eta$-nondegenerate. Given $m = \Omega(\lambda_2^{O(D)} \log(2n))$ i.i.d. samples from the RBM, where $D = O(\lambda_2 \log(\lambda_1 \lambda_2/\eta))$, we can recover its structure with high probability in time $poly(n^D)$.
\end{theorem}
Based on this result we also give a result for learning the RBM in TV distance under the same assumption: see Theorem~\ref{thm:dist-recovery-rbm}: the sample complexity of this method is essentially the above sample complexity plus $n^2 (1 - \tanh(\lambda_1))^{-d_2}$ where $d_2$ is the maximum 2-hop degree; the $poly(n)$ dependence is required as even learning $n$ bernoullis in TV requires $\Omega(n)$ sample complexity.

When interpreting these result, it is crucial not to confuse the $\ell_1$ norm parameters $\lambda_1,\lambda_2$ of visible and hidden units with the maximum degrees of these units. Typically in Ising models, we should think of the weight of a typical edge as \emph{shrinking} as $d$ grows so that units stay near the sensitive region of their activation and the behavior of the model does not become trivial --- this means that $\lambda_1$ and $\lambda_2$ may be much smaller than $d$. For example, probably the most well known sufficient condition for being able to sample in an Ising model (or RBM) is \emph{Dobrushin's uniqueness criterion} which is equivalent to the requirement that $\lambda_1,\lambda_2 \le 1$ and this condition is actually tight for Glauber dynamics to mix quickly in the Ising model on the complete graph (Curie-Weiss Model) \cite{levin2017markov}. We discuss this further in Remark~\ref{rmk:sampling-regimes}; as we explain there, in Dobrushin's uniqueness regime and under some mild nondegeneracy conditions we expect that $\eta = \Omega(1/d^2)$ so the above algorithm has runtime $n^{\log(d)}$, which is an exponential improvement in the exponent compared to the best previously known result ($O(n^d)$ runtime by viewing the RBM as an MRF).

We also give lower bound results showing that the computational complexity of the above algorithm is essentially optimal in terms of $\lambda_1$ and $\eta$ (based upon the hardness of learning sparse parity with noise) and nearly optimal in terms of $\lambda_2$ for an SQ (Statistical Query) algorithm, in the sense that any SQ algorithm needs at least sub-exponential dependence on $\lambda_2$ (given that the dependence on other parameters is not changed --- e.g. obviously there is a $2^n$ time algorithm to learn this problem). In particular, this shows that our results for learning feedforward networks under $\ell_{\infty}$ are close to tight even in this application, where the input distribution is related to the label.

%\paragraph{RBMs as a distributional assumption:} 
\paragraph{Supervised RBMs: } Since in many applications the input data to a classifier is clearly very structured (e.g. images, natural language corpuses, data on networks, etc.), it is interesting to consider the behavior of classification algorithms under structural assumptions on the data.
RBMs are one (relatively simple) generative model which can generate interesting structured data. This suggests the idea of learning ``supervised RBMs'', where we assume the input and label are drawn from an RBM joint distribution, so that predicting the label is a feedforward network by Theorem~\ref{thm:node-prediction-intro}; in this model the label is just a special visible unit in the RBM. Based on the previous discussion about computational lower bounds, we know that assuming the input to a feedforward network comes from the corresponding RBM does not in general make learning easier, but we know that in RBMs there are very natural assumptions we can make to avoid these computational issues. Our final result is of exactly this flavor, showing how we can learn the supervised RBM under a ferromagneticity-related condition faster than is possible if we did not have a distributional assumption.
%Our final result shows that under a structural assumptions on the RBM 
%(which also impose assumptions on the architecture of the feedforward network), assuming the data comes from the matching RBM \emph{can in fact} make learning the feedforward network computationally easier. 
%\subsubsection{Further Connections with Neural Networks}
% We believe that our approach gives a setting for neural network learning where structural properties of the input data are genuinely reasonable as well as useful.  \citep{?} \fnote{more discussion}.
%In other words, the connection between RBMs and Feedforward networks allows us to show how RBMs with certain structural assumptions can serve as a useful \emph{distributional assumption} for learning feedforward networks in a computationally efficient fashion. %We show that in a natural setting were the feedforward network is induced by a prediction task in an RBM, 
\begin{comment}
 This is done by using the relationship established in Theorem~\ref{thm:node-prediction} in the ``backwards'' direction, reducing from feedforward to RBM instead of RBM to feedforward. Under our structural assumptions, we can learn the feedforward network using structural properties of the RBM faster than is possible without this structural assumption.
\end{comment}

In order to emphasize the special role of the node which we want to predict, we will adopt a modified notation where the visible unit which we want to learn to predict is labeled $Y$ and all other visible units are still labeled $X$. More precisely, we model the joint distribution over input features $X$ valued in $\{\pm 1\}^{n_1}$, latent features $H$ valued in $\{ \pm 1\}^{n_2}$  and label $Y \in \{\pm 1\}$ as,
\[ \Pr[X = x,H = h,Y = y] \propto \exp\left(\langle x, Wh \rangle + \langle h, w\rangle y + \langle b^{(1)}, x \rangle + \langle b^{(2)}, h \rangle + b^{(3)}y\right) \]
where the \emph{weight matrix} $W$ is a non-negative $n_1 \times n_2$ matrix, $w$ is an arbitrary $n_1$ dimensional vector and \ $b^{(1)} \in \mathbb{R}^{n_2}$, $b^{(2)} \in \mathbb{R}^{n_2}$ and $b^{(3)} \in \mathbb{R}$ are arbitrary. Given the latent variables $H$, $w$ can be seen as the linear predictor for $Y$.

\begin{theorem}[Informal Version of Theorem \ref{thm:srbm_main}]\label{thm:smart-regression-intro}
Suppose the interaction matrix $W$ is ferromagnetic with minimum edge weight $\alpha$. Further suppose one of the RBMs induced by conditioning on $Y=1$ or $Y=-1$ is a $(\lambda, \lambda)$-RBM. Then there exists an algorithm that learns the predictor $Y$ that minimizes logistic loss up to erroe $\epsilon$. The algorithm has sample complexity $m = n_1^2\exp(\lambda)^{\exp(O(\lambda))}(1/\alpha)^{O(1)} \log(n_1/\delta)/\epsilon^2$ and has runtime $poly(m)$.
\end{theorem}
This result leverages tools from \citep{bresler2019learning,goel2019learning} but considers a setting where the RBM may in fact have some amount of negative correlation, as $w$ has arbitrary signs and is allowed to have large norm.
 Observe that under the given distributional assumptions, our algorithm has runtime complexity polynomial in the input dimension in contrast to Theorem \ref{thm:regression-intro} where the run time scales as $n^{\Omega(\lambda)}$.  A simple example which shows the algorithm from this Theorem will outperform any algorithm without distributional assumptions (like Theorem~\ref{thm:regression-intro}) is given in Remark~\ref{rmk:ferromagnetic-advantage}.

\subsection{Related Work on learning neural networks}\snote{This can probably go to the appendix.}
In the neural network learning literature, various works prove positive results that either (1) work for any distribution with norm assumptions or (2) require strong distributional assumptions. The result of Theorem~\ref{thm:regression-intro} falls into the category of (1) and the result of Theorem~\ref{thm:smart-regression-intro} falls generally into the category of (2).

We first discuss the relation of Theorem~\ref{thm:regression-intro} to other previous works of type (1). Perhaps the most closely related works are \cite{shalev2011learning,Zhang,goel2016reliably,goel2018learning}. All of these works assume the input is bounded in $\ell_2$ norm and give learning results based on kernel methods; of course, these results could be applied under the assumption of $\ell_{\infty}$-bounded input, by using the inequality $\|x\|_{2} \le \sqrt{n} \|x\|_{\infty}$ and rescaling the input to have norm $1$. For comparison, the best result in the $\ell_2$ setting with $\tanh$ activation is given in \cite{goel2018learning}, but this result (as is essentially necessary based on the known computational hardness results) has exponential dependence on the $\ell_2$ norm of the weights in the hidden units, so doing such a reduction just using norm comparison bounds gives a runtime sub-exponential in dimension. Therefore it is indeed crucial for us to give a new analysis adapting to learning with input bounded in $\ell_{\infty}$. An interesting feature of this setting (as mentioned above) is that the kernel trick does not seem to be as useful for improving the runtime as the $\ell_2$ setting, where it seems genuinely better than writing out the feature map \citep{goel2016reliably,goel2018learning}. 

%The work of \cite{Zhang} built upon \cite{shalev2011learning} and gave bounds for learning multilayer neural networks with kernel methods under the assumption that the $\ell_1$ norm of the network is bounded as well as the $\ell_2$ norm of the bottom layer and the input is normalized to have $\ell_2$ norm at most $1$. For a technical reason, they did not prove results for learning $\tanh$ networks but did give some results for networks with a somewhat similar $erf$ activation. Note that although they also assume $\ell_1$ bounds on the network, they crucially use the assumption that the input is bounded in $\ell_2$ 
%\fnote{todo}

Due to the generality of direction (1), it is hard to design efficient algorithms. This further motivates direction (2), however, making the right distributional assumptions which allow for efficient learning while being well-motivated in context of real world data can be very challenging. Most prior work has been limited to the Gaussian input \citep{tian2017analytical,soltanolkotabi2017learning,brutzkus2017globally,zhong2017recovery,li2017convergence,du2018gradient} or symmetric input \citep{goel2018learning,ge2019learning} assumptions which are not satisfied by real world data. The works of \cite{mossel2016deep,malach2018provably} gave results for some simple tree-structured generative models. There has been some work in defining data based notions such as eigenvalue decay \citep{goel2017eigenvalue} and score function computability \citep{gao2019learning} to get efficient results.  Our assumption for Theorem~\ref{thm:smart-regression-intro} in contrast exploits sparsity and nonnegative correlations among the input features conditional on the output label.


